Fault-tolerant qubit from a constant number of components

With gate error rates in multiple technologies now below the threshold required for fault-tolerant quantum computation, the major remaining obstacle to useful quantum computation is scaling, a challenge greatly amplified by the huge overhead imposed by quantum error correction itself. We propose a fault-tolerant quantum computing scheme that can nonetheless be assembled from a small number of experimental components, potentially dramatically reducing the engineering challenges associated with building a large-scale fault-tolerant quantum computer. Our scheme has a threshold of 0.39% for depolarising noise, assuming that memory errors are negligible. In the presence of memory errors, the logical error rate decays exponentially with $\sqrt{T/\tau}$, where $T$ is the memory coherence time and $\tau$ is the timescale for elementary gates. Our approach is based on a novel procedure for fault-tolerantly preparing three-dimensional cluster states using a single actively controlled qubit and a pair of delay lines. Although a circuit-level error may propagate to a high-weight error, the effect of this error on the prepared state is always equivalent to that of a constant-weight error. We describe how the requisite gates can be implemented using existing technologies in quantum photonic and phononic systems. With continued improvements in only a few components, we expect these systems to be promising candidates for demonstrating fault-tolerant quantum computation with a comparatively modest experimental effort.

==> latticediagram.tex <==
\tdplotsetmaincoords{70}{120} % set viewpoint 
\tdplotsetrotatedcoords{10}{-90}{90} %<- rotate around (z,y,z)
\newboolean{bodycenterline}
\begin{tikzpicture}[scale=1.3,tdplot_rotated_coords,
                    rotated axis/.style={->,purple,ultra thick},
                    blackBall/.style={ball color = black!80},
                    borderBall/.style={ball color = white,opacity=.25}, 
                    very thick]

\foreach \x in {0,1,2,3,4}
    \foreach \y in {1,2,3,4,5}
        \foreach \z in {0,1,2}{

           %#####################################################
           \ifthenelse{ \NOT \(\equal{\intcalcMod{\z}{2}}{1} \AND \equal{\intcalcMod{\y}{2}}{1}\) \AND \(\x<4\)}{
             \ifthenelse{\equal{\intcalcMod{\z+\y}{2}}{0}} {
                 \draw [help lines] (\x,\y,\z) -- (\x+1,\y,\z);
             }{
                 \draw [thick,line cap=round,opacity=1-\z/2.5] (\x,\y,\z) -- (\x+1,\y,\z);
             }
           }{}
           %#####################################################
           \ifthenelse{ \NOT \(\equal{\intcalcMod{\x}{2}}{1} \AND \equal{\intcalcMod{\z}{2}}{1}\) \AND \(\y<5\)}{
               \ifthenelse{\equal{\intcalcMod{\x+\z}{2}}{0}} {
                   \draw [help lines] (\x,\y,\z) -- (\x,\y+1,\z);
               }{
                   \draw [thick,line cap=round,opacity=1-\z/2.5] (\x,\y,\z) -- (\x,\y+1,\z);
               }
           }{}
           %#####################################################
           \ifthenelse{ \NOT \(\equal{\intcalcMod{\x}{2}}{1} \AND \equal{\intcalcMod{\y}{2}}{1}\) \AND \(\z<2\)}{
               \ifthenelse{\equal{\intcalcMod{\x+\y}{2}}{0}}{
                   \draw [help lines] (\x,\y,\z) -- (\x,\y,\z+1);
               }{
                   \draw [thick,line cap=round,opacity=1-\z/2.5] (\x,\y,\z) -- (\x,\y,\z+1);
               }
           }{}
}

% axes
\draw [mycyan,->,opacity=0.7] (0,0+1,0) -- (0,0+1,4);
\node [above,mycyan] at (0,0+1,4) {$z$};
\draw [mycyan,->,opacity=0.7] (0,0+1,0) -- (0,5+1,0);
\node [left,mycyan] at (0,5+1,0) {$y$};
\draw [mycyan,->,opacity=0.7] (0,0+1,0) -- (5.3,0+1,0);
\node [right,mycyan] at (5.3,0+1,0) {$x$};



\foreach \x in {0,1,2,3,4}
   \foreach \y in {1,2,3,4,5}
      \foreach \z in {0,1,2}{
          \ifthenelse{
              \NOT \( \equal{\intcalcMod{\x}{2}}{\intcalcMod{\y}{2}} \AND \equal{\intcalcMod{\y}{2}}{\intcalcMod{\z}{2}} \)
          }{
              \shade[rotated axis,blackBall,opacity=1-\z/2.5] (\x,\y,\z) circle (0.1cm);
          }{}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% (QUBIT LABELS -- let me know if you need help -noah)
%  _____  _     _ ______  _____ _______             _______ ______  _______        _______
% |   __| |     | |_____]   |      |         |      |_____| |_____] |______ |      |______
% |____\| |_____| |_____] __|__    |         |_____ |     | |_____] |______ |_____ ______|
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% qubit labels
% (0,1,0) is the (x,y,z) origin
\node [above left,black] at (0,1,0) {$1$};
\node [above left,black] at (1,1,0) {$2$};
\node [above left,black] at (2,1,0) {$3$};
\node [above left,black] at (3,1,0) {$4$};
\node [above left,black] at (4,1,0) {$5$};
\node [above left,black] at (1,2,0) {$7$};
\node [above left,black] at (3,2,0) {$9$};
\node [above left,black] at (0,3,0) {$11$};
\node [above left,black] at (1,3,0) {$12$};
\node [above left,black] at (2,3,0) {$13$};
\node [above left,black] at (3,3,0) {$14$};
\node [above left,black] at (4,3,0) {$15$};
\node [above left,black] at (1,4,0) {$17$};
\node [above left,black] at (3,4,0) {$19$};
\node [above left,black] at (0,5,0) {$21$};
\node [above left,black] at (1,5,0) {$22$};
\node [above left,black] at (2,5,0) {$23$};
\node [above left,black] at (3,5,0) {$24$};
\node [above left,black] at (4,5,0) {$25$};
\node [above left,black] at (0,1,1) {$26$};
\node [above left,black] at (2,1,1) {$28$};
\node [above left,black] at (4,1,1) {$30$};
%\node [right,opacity=0.8,black] at (2,1,2) {$\ell$};
%\node [right] at (4,4+1,2) {favorite qubit};
%\node [right] at (4,2+1,1) {least favorite qubit};
%\node [below] at (2,5+1,1) {special  qubit};
%\draw [->] (2,5+1,1) -- (1.1,4.1+1,0);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\end{tikzpicture}

==> unitcell.tex <==
\tdplotsetmaincoords{70}{120} % set viewpoint 
\tdplotsetrotatedcoords{10}{-90}{90} %<- rotate around (z,y,z)
\newboolean{bodycenterline}
\begin{tikzpicture}[scale=1.3,tdplot_rotated_coords,
                    rotated axis/.style={->,purple,ultra thick},
                    blackBall/.style={ball color = black!80},
                    borderBall/.style={ball color = white,opacity=.25}, 
                    very thick]

\foreach \x in {0,1,2}
    \foreach \y in {0,1,2}
        \foreach \z in {0,1,2}{

           %#####################################################
           \ifthenelse{ \NOT \(\equal{\intcalcMod{\z}{2}}{1} \AND \equal{\intcalcMod{\y}{2}}{1}\) \AND \(\x<2\)}{
             \ifthenelse{\equal{\intcalcMod{\z+\y}{2}}{0}} {
                 \draw [help lines] (\x,\y,\z) -- (\x+1,\y,\z);
             }{
                 \draw [thick,line cap=round,opacity=1-\z/2.5] (\x,\y,\z) -- (\x+1,\y,\z);
             }
           }{}
           %#####################################################
           \ifthenelse{ \NOT \(\equal{\intcalcMod{\x}{2}}{1} \AND \equal{\intcalcMod{\z}{2}}{1}\) \AND \(\y<2\)}{
               \ifthenelse{\equal{\intcalcMod{\x+\z}{2}}{0}} {
                   \draw [help lines] (\x,\y,\z) -- (\x,\y+1,\z);
               }{
                   \draw [thick,line cap=round,opacity=1-\z/2.5] (\x,\y,\z) -- (\x,\y+1,\z);
               }
           }{}
           %#####################################################
           \ifthenelse{ \NOT \(\equal{\intcalcMod{\x}{2}}{1} \AND \equal{\intcalcMod{\y}{2}}{1}\) \AND \(\z<2\)}{
               \ifthenelse{\equal{\intcalcMod{\x+\y}{2}}{0}}{
                   \draw [help lines] (\x,\y,\z) -- (\x,\y,\z+1);
               }{
                   \draw [thick,line cap=round,opacity=1-\z/2.5] (\x,\y,\z) -- (\x,\y,\z+1);
               }
           }{}
}

% % axes
% \draw [blue,->,opacity=0.5] (0,0+1,0) -- (0,0+1,4);
% \node [above,blue] at (0,0+1,4) {$z$};
% \draw [blue,->,opacity=0.5] (0,0+1,0) -- (0,5+1,0);
% \node [left,blue] at (0,5+1,0) {$y$};
% \draw [blue,->,opacity=0.5] (0,0+1,0) -- (5,0+1,0);
% \node [right,blue] at (5,0+1,0) {$x$};



\foreach \x in {0,1,2}
   \foreach \y in {0,1,2}
      \foreach \z in {0,1,2}{
          \ifthenelse{
              \NOT \( \equal{\intcalcMod{\x}{2}}{\intcalcMod{\y}{2}} \AND \equal{\intcalcMod{\y}{2}}{\intcalcMod{\z}{2}} \)
          }{
              \shade[rotated axis,blackBall,opacity=1-\z/2.5] (\x,\y,\z) circle (0.1cm);
          }{}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% (QUBIT LABELS -- let me know if you need help -noah)
%  _____  _     _ ______  _____ _______             _______ ______  _______        _______
% |   __| |     | |_____]   |      |         |      |_____| |_____] |______ |      |______
% |____\| |_____| |_____] __|__    |         |_____ |     | |_____] |______ |_____ ______|
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% qubit labels
% (0,1,0) is the (x,y,z) origin
% \node [above left,red] at (0,1,0) {$1$};
% \node [above left,red] at (1,1,0) {$2$};
% \node [above left,red] at (2,1,0) {$3$};
% \node [above left,red] at (3,1,0) {$4$};
% \node [above left,red] at (4,1,0) {$5$};
% \node [above left,red] at (1,2,0) {$7$};
% \node [above left,red] at (3,2,0) {$9$};
% \node [above left,red] at (0,3,0) {$11$};
% \node [above left,red] at (1,3,0) {$12$};
% \node [above left,red] at (2,3,0) {$13$};
% \node [above left,red] at (3,3,0) {$14$};
% \node [above left,red] at (4,3,0) {$15$};
% \node [above left,red] at (1,4,0) {$17$};
% \node [above left,red] at (3,4,0) {$19$};
% \node [above left,red] at (0,5,0) {$21$};
% \node [above left,red] at (1,5,0) {$22$};
% \node [above left,red] at (2,5,0) {$23$};
% \node [above left,red] at (3,5,0) {$24$};
% \node [above left,red] at (4,5,0) {$25$};
% \node [above left,red] at (0,1,1) {$26$};
% \node [above left,red] at (2,1,1) {$27$};
%\node [right,opacity=0.8,red] at (2,1,2) {$\ell$};
%\node [right] at (4,4+1,2) {favorite qubit};
%\node [right] at (4,2+1,1) {least favorite qubit};
%\node [below] at (2,5+1,1) {special  qubit};
%\draw [->] (2,5+1,1) -- (1.1,4.1+1,0);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\end{tikzpicture}
